Dynamic DAG-Application Scheduling for Multi-Tier Edge Computing in Heterogeneous Networks

Edge computing is deemed a promising technique to execute latency-sensitive applications by offloading computation-intensive tasks to edge servers. Extensive research has been conducted in the field of end-device to edge server task offloading for several goals, including latency minimization, energy optimization, and resource optimization. However, few of them consider our mobile computing devices (smartphones, tablets, and laptops) to be edge devices. In this paper, we propose a novel multi-tier edge computing framework, which we refer to as M-TEC, that aims to optimize latency, reduce the probability of failure, and optimize cost while accounting for the sporadic failure of personally owned devices and the changing network conditions. We conduct experiments with a real testbed and a real commercial CBRS 4G network, and the results indicate that M-TEC is capable of reducing the end-to-end latency of applications by at least 8\% compared to the best baseline under a variety of network conditions, while providing reliable performance at an affordable cost.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> author_bio.tex <==
\section{Author Biography}
\vspace{-10 mm}
\begin{IEEEbiographynophoto}{Xiang Li}
(li2068@purdue.edu)
Ph.D. student in ECE at Purdue University
\vspace{-10 mm}
\begin{IEEEbiographynophoto}{Mustafa Abdallah}
(abdalla0@purdue.edu)
Assistant Professor of CIT at Purdue University
\vspace{-10 mm}
\begin{IEEEbiographynophoto}{Yuan-Yao Lou}
(lou45@purdue.edu)
Ph.D. student in ECE at Purdue University
\vspace{-10 mm}
\begin{IEEEbiographynophoto}{Mung Chiang}
(chiang@purdue.edu)
is President of Purdue University.
\end{IEEEbiographynophoto}
\vspace{-10 mm}
\begin{IEEEbiographynophoto}{Kwang Taik Kim}
(kimkt@purdue.edu)
is Research Assistant Professor of ECE at Purdue University
\vspace{-10 mm}
\begin{IEEEbiographynophoto}{Saurabh Bagchi}
(sbagchi@purdue.edu)
is Professor of ECE at Purdue University


==> todo.tex <==
1. Find a real-world application to back up our motivation.
 - I added BitTorrent as an example application. MTEC is like a more generalized BitTorrent that is capable of dynamically scheduling tasks on peer machines within its network. (rephrase and find another example) {- fixed}

2. Fix the grammar in our sentence for the DAG explanation.
 - fixed

3. Mention that fairness is not covered in the paper.
 -  In section 3.4, added that there exists rich literature in fairness scheduling in edge and cloud computing(cited 4 papers from this topic). Then we mentioned that fairness is not the focus of this paper but it can be easily enforced by the initiator during the orchestration stage.

4. Explicitly describe the peak load observed in our experiments in the paper.
 - By repeating the experiments multiple times, we are able to retrieve the average performance of the orchestration scheme as well as exam the performance under randomly generated peak load.

5. In terms of profiling details, please provide a brief description and cite our previous paper.

 - Added more details into section 3.3 {Note that a device will not be considered as the candidate of the orchestration network until its profiling is finished. Once the device is profiled, its profiling data will be shared with other devices in the network to avoid redundant profiling.} and cited our SRDS paper.


6. "Section 3.4 addresses the scalability issue by letting the initiator divide the network based on proximity, and we define the proximity as the round trip time," support this claim with references or our analysis and figures.

- in section 3.4 scalibility paragraph last sentence, I cited two more papers as {Similar approaches are used by \cite{cluster_head1, cluster_head2}. Instead of using round trip time to measure proximity, they use devices with localization capability as gateways to manage other devices on the same local area network.} {the idea of dividing...into is shared by ..., however.. } { - fixed}
